Optimization Strategies for Real-Time Control of an Autonomous Melting Probe

We present an optimization-based approach for trajectory planning and control of a maneuverable melting probe with a high number of binary control variables. The dynamics of the system are modeled by a set of ordinary differential equations with a priori knowledge of system parameters of the melting process. The original planning problem is handled as an optimal control problem. Then, optimal control is used for reference trajectory planning as well as in an MPC-like algorithm. Finally, to determine binary control variables, a MINLP fitting approach is presented. The proposed strategy has recently been tested during experiments on the Langenferner glacier. The data obtained is used for model improvement by means of automated parameter identification.

==> statement.tex <==
\section{Introduction}

During the Cassini-Huygens mission, lasting for nearly 20 years and coming to an end by September 2017, the Saturnian moon Enceladus has been found to be one of the most interesting celestial bodies in our solar system regarding future exploration missions.
Plumes that ascend from the south polar region could be detected by the Cassini spacecraft and were identified to contain ionized water vapor. Additionally, camera recordings showed large scrapes in Enceladus' kilometers thick icy shell with elevated surface temperatures, the so-called ``Tiger stripes''. 
Evaluations of the gathered information indicate cryovolcanism as the reason for such activity with the consequence that there is a global liquid water ocean below the surface \cite{porco2006cassini}. The possibility of proving extraterrestrial life in it or habitability were a starting signal for several mission concepts.\par 
One of these ideas has been developed during the Enceladus Explorer (``EnEx'') collaborative project. A possible scenario would be to retrieve water samples from the ocean by drilling through the icy shell. If aiming for cracks close to the geysers and hitting liquid water reservoirs, the mission objective could be accomplished  relatively easy. 
Therefore, a maneuverable melting probe has been built, the IceMole \cite{dachwald2014icemole} (Fig. \ref{fig:icemole}).
\begin{figure}[ht]
	\centering
	\includegraphics{pictures/icemole.pdf}
	\caption{IceMole during the 2013 Morteratsch field test}
	\label{fig:icemole}
\end{figure}  
During several field tests it's ability to locate itself and to maneuver trough ice has been shown. A scientific highlight was the first successful retrieving of a clean brine sample of the Blood Falls in Antarctica \cite{kowalski2016navigation}. 
After demonstrating the general technical feasibility of the mission concept, necessary technologies shall now be further enhanced in six following research projects, each focusing on different parts.
In EnEx-CAUSE a fully autonomous navigation system is being developed, implying  sensor fusion, decision making and steering the probe. \par The challenge of guiding the IceMole includes a sequence of tasks. From modeling the system dynamics over trajectory planning to determining the actuator controls, a coherent concept is required. Optimization methods can be a useful strategy to solve each of these problems and additionally allow easy transferability. As a consequence all packages can be deduced to optimal control problems (OCP) or respectively, because of the binary character of the heater units, to mixed-inter control problems (MIOCP). For solving these, there exists no universal best approach but a variety of strategies. We propose a pragmatic concept that at some point neglects dynamics exactness, but guarantees a solution under real-time conditions. 
\subsection{Related Work}
The studying of OCPs became popular in the 1950s and 1960s when there was a high demand for solutions in the military sector \cite{sussmann1997300}. Solution strategies can be divided into two classes of approaches \cite{stryk1992direct}. Direct methods transcribe the problem by collocation, multiple shooting or full discretization methods into nonlinear programs (NLP). These potentially high-dimensional problems can be solved by sequential quadratic programming or interior point algorithms. The indirect approach uses Pontryagin's maximum principle to form the necessary optimality conditions which leads to a boundary value problem that again can be solved by shooting methods. MIOCPs or often also referred als hybrid optimal control problems have firstly been studied in the 1980s. They are considered to be much harder to solve than pure OCPs \cite{kirches2011fast}. Similarly, they can be deduced to mixed-integer nonlinear programs (MINLP), which typically are solved by branch-and-bound algorithms. Otherwise, there exist alternative and often combined strategies including relaxation, transformation or rounding techniques, e.g. as in \cite{gerdts2006variable} \cite{sager2005numerical}.


